Competition-Based Resilience in Distributed Quadratic Optimization

This paper proposes a novel approach to resilient distributed optimization with quadratic costs in a networked control system (e.g., wireless sensor network, power grid, robotic team) prone to external attacks (e.g., hacking, power outage) that cause agents to misbehave. Departing from classical filtering strategies proposed in literature, we draw inspiration from a game-theoretic formulation of the consensus problem and argue that adding competition to the mix can enhance resilience in the presence of malicious agents. Our intuition is corroborated by analytical and numerical results showing that i) our strategy highlights the presence of a nontrivial tradeoff between blind collaboration and full competition, and ii) such competition-based approach can outperform state-of-the-art algorithms based on Mean Subsequence Reduced.

==> Sections/conclusion.tex <==
%!TEX ROOT = ../collaboration_vs_competition.tex

\section{Conclusion}\label{sec:conclusion}

In this paper,
we have proposed a competitive approach
to tame adversarial attacks in networked systems.
We have presented analytical and numerical insights on its performance,
showed that it can outperform classical resilient consensus algorithms,
and discussed directions for future research.

==> Sections/discussion-optimization.tex <==
%!TEX ROOT = ../collaboration_vs_competition.tex

\section{Discussion: Optimization of the FJ Dynamics}\label{sec:discussion-optimization}

In the previous sections,
we discussed the benefit of using a game-theoretic approach such as FJ dynamics
to mitigate the effect of malicious \nodes in reaching consensus and solving a distributed optimization task.
While the theoretical results presented in~\autoref{sec:malicious}
and the numerical experiments provided in~\autoref{sec:numerical-tests-FJ-err}
prove that indeed such a design is beneficial to the optimization enhancing robustness,
choosing optimally the parameter $ \lam $ is an issue.
Indeed, the points of minimum of the error curves plotted in~\autoref{sec:numerical-tests-FJ-err}
can be computed only if the malicious \nodes were known.
In fact, while it may be true that for some particular cases
(\eg regular graphs, sparse networks)
the identity of malicious \nodes has null or negligible impact,
in general the shape of the cost function~\eqref{eq:cons-error-regular}
changes according to both quantity and position of the malicious \nodes.

Clearly, in a real setup, the identity of malicious \nodes is unknown,
which requires to compute $ \lam^* $ based on heuristics or approximate solutions.
In words, one would like to design $ \lam $ without knowing the identity of malicious \nodes,
while trying to maximize some reasonable performance metric.
A naive approach is to optimize the worst-case scenario,
where the malicious \nodes cause the highest damage:
\begin{equation}\label{eq:optimization-worst-case}
	\min_{\lam}\max_{\malSet:\lvert\malSet\rvert=M} \E{\left\|\xreg(\lam;\malSet)-\one_R\thbarreg\right\|^2}.
\end{equation}
In~\eqref{eq:optimization-worst-case},
we have highlighted that the optimization variables affect only the steady state $ x_\regSet $,
and further imposed the amount of malicious \nodes $ M $ to make the problem well posed.
Notice that, if $ M = 1 $, such a worst-case design can be carried out with linear complexity in the number of \nodes $ N $,
by parsing all \nodes to see which one yields the largest error
and then minimizing its associate error curve.
This latter stage can be performed via gradient- or Newton-like descent,
or even with brute-force search by discretizing over $ \lam $.
Conversely, with generic $ M > 1 $,
the exact solution of~\eqref{eq:optimization-worst-case} requires a combinatorial search
whose complexity grows exponentially with $ M $,
and is thus intractable if many malicious \nodes are assumed
and/or with large-scale networks.

In light of the above considerations,
we leave the study of $ \lam $-optimization as future work.
Specifically, we aim to target the following questions.
\begin{itemize}
	\item Is it possible to (approximately) solve~\eqref{eq:optimization-worst-case} in polynomial time?
		There exist graphs for which~\eqref{eq:optimization-worst-case} can be solved in polynomial time?
	\item What is the suboptimality gap of~\eqref{eq:optimization-worst-case} with respect to the true $ \lam^* $
		(\ie minimizing the true error with the actual malicious \nodes)?
	\item Are there smarter choices of $ \lam^* $ than worst-case design, which may require,
		\eg online and/or decentralized/distributed adaptation, possibly with a different $ \lam_i $ for each \node $ i $?
\end{itemize}

==> Sections/network-optimization.tex <==
%!TEX ROOT = ../collaboration_vs_competition.tex

\section{Network Optimization}\label{sec:network-optimization}

In the previous sections,
we discussed the benefits of using a game-theoretic approach -- such as FJ dynamics --
to mitigate the effect of malicious \nodes in solving a distributed optimization task.
Grounding on this competitive dynamics,
we now shift our attention to the analysis of network topology
%(if possible)
in order to further improve system performance and robustness.

Apart from the consensus error dealt with so far,
we also evaluate system controllability by the malicious \node
as explained next.
Consider the following rewriting of~\eqref{eq:FJ-dynamics},
\begin{equation}\label{eq:FJ-dynamics-input-malicious}
	\xreg(k+1) = (1-\lam)\Wreg\xreg(k) + \lam\theta_\regSet + (1-\lam)\Wm\xm(k),
\end{equation}
where $ \Wreg $ corresponds to interactions among regular \nodes,
$ \Wm $ to the neighbors of the malicious \node
and for the sake of simplicity we assume a single malicious, \ie $ \malSet = \{m\} $.
\cref{eq:FJ-dynamics-input-malicious} can be interpreted as a controlled system
where the control input is the malicious \node's state,
and the priors of regular \nodes act as exogenous inputs.
A performance metric related to the control effort
in~\eqref{eq:FJ-dynamics-input-malicious}
is quantified by the controllability Gramian,
\begin{equation}\label{eq:gramian}
		\Gram{K} = (1-\lam)^2\sum_{k=0}^{K-1}(1-\lam)^{2k}\Wreg^k\Wm\Wm^\top\left(\Wreg^\top\right)^k,
\end{equation}
where we choose $ K $ as the reachability index.
In particular, the trace of $ \Gram{K} $ 
(in the following referred to as \emph{controllability index})
is inversely related to the average control energy spent in $ K $ steps,
and has been used in several works in literature~\cite{gramian}.
Hence, a small value for $ \tr{\Gram{K}} $ means that the malicious \node
can steer the regular \nodes with high energy consumption
(averaged over the reachable set),
which may be a desirable feature to drain out adversarial resources.
Further, as the controllability index can be written as
\begin{equation}\label{eq:trace-gramian}
	\tr{\Gram{K}} = (1-\lam)^2\sum_{k=0}^{K-1}\Big\|(1-\lam)^{k}\Wreg^k\Wm \Big\|^2,
\end{equation}
%we note that 
it shares some resemblance with the component $ e_{\regSet,\mathrm{collaboration}} $ of the consensus error,
which is proportional to (cf.~\eqref{eq:cons-error-regular-split})
\begin{equation}\label{eq:cons-error-rewritten}
	\begin{aligned}
		\left\| L_m^{-m}\right\|^2 &= \Bigg\|\sum_{k=0}^{\infty}(1-\lam)^k\selreg W^ke_m \Bigg\|^2\\
								   &= \Bigg\|\sum_{k=0}^{\infty}(1-\lam)^k\sum_{j=0}^{k-1}\Wreg^j\Wm \Bigg\|^2.
	\end{aligned}
\end{equation}
In particular, both $ \tr{\Gram{K}} $ and $ e_{\regSet,\mathrm{collaboration}} $ are decreasing with $ \lam $
and depend on the vectors $ \Wreg^k\Wm $,
which describe the effect of the malicious \node over the rest of the network after $ k $ steps.
Also, even though $  e_{\regSet,\mathrm{collaboration}} $ involves an infinite summation,
the discount factor $ (1-\lam)^k $ makes the tail negligible,
inducing resemblance with the controllability index.
\begin{rem}[Controllability from Malicious Agent]
	Notice that the controllability index allows to consider a richer behavior
	of the malicious \node,
	which can exploit a time-varying state to drive the regular \nodes to any values
	in the reachable set.
\end{rem}

In light of the above observation,
we consider the following optimization problems,
\begin{gather}
	\min_{W}\max_{m\in\sensSet} \;\; \ereg, \label{eq:optimization-network-err} \tag{PE}\\
	\min_{W}\max_{m\in\sensSet} \;\; \tr{\Gram{K}}. \label{eq:optimization-network-contr} \tag{PC}
\end{gather}
The internal maximization reflects a worst-case design:
in~\eqref{eq:optimization-network-err}, the malicious \node is selected as the \node
leading to the largest consensus error,
while in~\eqref{eq:optimization-network-contr} it is chosen as the one
with most powerful controllability,
quantified as low average energy consumption.
The external minimization is the network design,
aimed to either decrease the consensus error~\eqref{eq:optimization-network-err}
or to increase the energy consumption~\eqref{eq:optimization-network-contr}.

The above problems are not convex, in general.
Further, the internal maximization over \node set
makes it hard to frame them in standard optimization frameworks,
because it requires to parse all \nodes for each choice of $ W $.
Hence, heuristics are needed to find suboptimal solutions.
%Clearly, designing a generic (weighted) graph $ W $ is a combinatorial problem
%which becomes intractable as the network size grows.

\begin{figure}
	\centering
	\begin{minipage}[l]{.5\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/Graph/Regular/err_cost_deg_3-10_N_100_it_1000_lam_0,1_d_100}
	\end{minipage}%
	\begin{minipage}[r]{.5\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/Graph/Regular/contr_index_deg_3-10_N_100_it_1000_lam_0,1}
	\end{minipage}
	\caption{Average consensus error (left) and controllability index (right) for $ 100 $-node regular graphs with uniform weights, with $ \lam = 0.1 $.}
%		with degree ranging from $ 3 $ to $ 10 $.
	\label{fig:net-opt-regular}
\end{figure}

As a first step to make the optimization more tractable,
we restrict ourselves to regular graphs with uniform weights.
%and compare different node degrees.
\autoref{fig:net-opt-regular} shows the considered performance metrics computed for
regular graphs with different degrees, % ranging from $ 3 $ to $ 10 $,
obtained by averaging over $ 1000 $ random graphs for each degree.
The~\textquotedblleft worst" malicious \node was found by
brute-force search on each graph.

A first insight is that
increasing the graph connectivity mitigates adversarial attacks,
from both consensus and energy consumption standpoints.
This is intuitive as, while all graphs are edge-wise balanced,
the malicious \node faces a larger number of uncontrolled interactions
as the degree increases.

\begin{algorithm}
	\caption{Greedy Edge Removal}
	\label{alg:greedy-removal}
	\begin{algorithmic}[1]
		\Require $ \Delta $-regular graph $ W $, $ \lam $, amount of edges to be removed $ E_{\text{rm}} $, performance metric $ c\in\{\ereg,\tr{\Gram{K}}\} $.
		\Ensure Graph $ W $ with $ E_{\text{rm}} $ less edges s.t. each node has degree in $ \{\Delta-1,\Delta\} $.
		\While{not removed $ E_{\text{rm}} $ edges}
			\State $ \mathcal{E}_{\text{curr}} \leftarrow $ candidate edges for removal;
%				such that incident nodes have degree $ \Delta $;
			\ForAll{$ e \in \mathcal{E}_{\text{curr}} $}
%				\State $ \mathcal{E}_{\text{tmp}} \leftarrow \mathcal{E}_{\text{curr}} \setminus \{e\}$;
				\State $ W_{\text{tmp}} \leftarrow $ remove $ e $ from $ W $ and re-weigh; % affected neighborhoods (uniform weights);
				\State $ c_e \leftarrow \max_{m\in\sensSet} \;\; c(W_{\text{tmp}}) $;
			\EndFor
			\State $ e^* \leftarrow \argmin_e c_e $;
			\State $ W \leftarrow $ remove $ e^* $ from $ W $ and re-weigh; % affected neighborhoods (uniform weights);
		\EndWhile
	\end{algorithmic}
\end{algorithm}

%Moreover,
%~\autoref{fig:net-opt-regular} suggests that the graph connectivity
%should be increased as much as possible to exploit regular \nodes cooperation.
In real systems, the number of communication links is bounded by practical constraints.
%Leveraging the intuition that balanced graphs should perform better,
We next refine the coarse regular-graph network design as follows:
given an upper bound on the overall number of links in terms of a $ \Delta $-regular graph,
we gradually remove edges so as to minimize the performance degradation.
More specifically, given $ W $,
we iteratively remove the edge which solves~\eqref{eq:optimization-network-err} or~\eqref{eq:optimization-network-contr}
where the minimization is restricted to an edge in the graph (couple of rows in $ W $),
with the further constraint that at most one edge be removed per node.
The latter condition %allows us to explore how the cost indices vary
%between any two consecutive points in~\autoref{fig:net-opt-regular},
keeps the \node' degrees as balanced as possible:
this allows us to explore how performance varies
between any two consecutive points in~\autoref{fig:net-opt-regular}.
%(possibly) reaching a $ (\Delta-1) $-regular graph. % from a $ \Delta $-regular graph,
%which is useful to compare regular and non-regular architectures.
Further, such a greedy removal is motivated by numerical tests showing that, in non-regular graphs,
the adversary exploits higher-connected \nodes to make more damage.
However, the greedy algorithm may not remove \emph{exactly} one edge per node, in general.
In fact, it is possible to obtain a $ (\Delta-1) $-regular graph
by pruning a $ \Delta $-regular graph 
only if the latter admits a \emph{perfect matching},
and in this case a solution is to remove all edges in such a matching.%
\footnote{A matching is a subset of edges which do not share nodes.
	A maximum matching is a matching of maximal cardinality, and a perfect matching is a maximum matching whose edges touch all nodes.}
The procedure is outlined in~\cref{alg:greedy-removal}.

\begin{rem}[Greedy Removal \textit{vs} Addition]
	An alternative %to greedily removing edges from a $ \Delta $-regular graph
	is to greedily adding edges to a $ (\Delta-1) $-regular graph.
	However, this is more computationally expensive because the amount of candidate edges
	to be evaluated at each iteration is in $ O(N^2) $,
	while the greedy removal requires only $ O(N) $ evaluations.
\end{rem}
\begin{rem}[Amount and Sub-optimality of Removed Edges]
	We assume that the amount of edges to be removed by the greedy algorithm, $ E_{\text{rm}} $,
	is compatible with the minimal maximum matching of the graph,
	so that the procedure terminates correctly.
	In general, the degree constraint in~\cref{alg:greedy-removal} may be relaxed
	to allow for removing an arbitrary amount of edges.
	We do not assess the impact of such a constraint
	because we are interested in understanding how the performance varies
	when shifting from $ \Delta $-regular to $ (\Delta-1) $-regular graphs.
	More in general, the algorithm could be improved to work with general graphs,
	but this goes beyond the scope of this paper.
\end{rem}

\begin{figure}
	\centering
	\begin{minipage}[l]{.5\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/Graph/Non-regular/err_deg_4to3_N_50_d10_lam_0,7}
	\end{minipage}%
	\begin{minipage}[r]{.5\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/Graph/Non-regular/contr_ind_4to3_N_50_d10_lam_0,7}
	\end{minipage}
	\caption{Consensus error (left) and controllability index (right) with greedy edge removal 
		starting from a $ 4 $-regular graph ($ 100 $ edges), with $ \lam = 0.7 $.}
	\label{fig:net-opt-non-regular-lam-0.7}
\end{figure}
\begin{figure}
	\centering
	\begin{minipage}[l]{.5\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/Graph/Non-regular/err_deg_4to3_N_50_d10_lam_0,2}
	\end{minipage}%
	\begin{minipage}[r]{.5\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/Graph/Non-regular/contr_ind_4to3_N_50_d10_lam_0,2}
	\end{minipage}
	\caption{Consensus error (left) and controllability index (right) with greedy edge removal 
		starting from a $ 4 $-regular graph ($ 100 $ edges), with $ \lam = 0.2 $.}
	\label{fig:net-opt-non-regular-lam-0.2}
\end{figure}

Figures~\ref{fig:net-opt-non-regular-lam-0.7}--\ref{fig:net-opt-non-regular-lam-0.2}
show the performance obtained by the greedy algorithm starting from a $ 4 $-regular graph,
%(right end of $ x $-axis),
together with the performance attained by $ 3 $-regular graphs
obtained by removing a perfect (maximum) matching. % (left end of $ x $-axis).
The first notable thing is that,
for both indices,
the performance degrades (almost) monotonically as edges are removed (from right to left on the $ x $-axis). % up to a certain point of maximum,
This may be explained by a combination of lower connectivity,
as remarked above, and graph unbalance,
which hinders the ideal \textquotedblleft democratic" collaboration across regular \nodes
and allows the adversarial to exploit higher-connected malicious \nodes against low-connected regular \nodes.

Secondly, while the consensus error increases quite smoothly,
the controllability index exhibits sharper \textquotedblleft jumps".
This is true in particular when $ \lam $ is larger (see~\autoref{fig:net-opt-non-regular-lam-0.7}),
as it makes the system more stable w.r.t. the topology.
Such a behavior suggests the presence of groups of edges which are critical to performance,
and may help in deciding which communication links should be kept or can be removed.

Further, in almost all tests,
the $ 3 $-regular graph obtained by removing a perfect matching
yielded a performance improvement compared to the last greedy iteration
(left-most blue diamond),
see~\autoref{fig:net-opt-non-regular-lam-0.7}.
This is insightful as it shows that increasing connectivity may not be beneficial
if it entails a loss in the degree balance:
in~\autoref{fig:net-opt-non-regular-lam-0.7}, the $ 3 $-regular graph induced by the perfect matching
reduces the controllability index by $ 22\% $ w.r.t.
the last algorithm iteration (a $ 3 $-regular graph plus one edge),
and has comparable performance with graphs having more than $ 90 $ edges.
This suggests a phase transition in the network design,
where it is not convenient to add edges until a certain threshold.
However,
as shown in~\autoref{fig:net-opt-non-regular-lam-0.2},
a perfect matching %(which has no relation to the greedy algorithm)
may yield much worse performance than even the more unbalanced graphs
that are obtained by running the greedy algorithm.
This gives a further insight: removing an arbitrary edge subset
may not yield the expected advantage, unless chosen according to some suitable criteria.
In fact, $ 3 $-regular graphs obtained from the greedy algorithm
\emph{always} outperformed the last non-regular iteration(s).


==> Sections/simulations.tex <==
%!TEX ROOT = ../collaboration_vs_competition.tex

\section{Numerical simulations}\label{sec:simulations}

Very convincing simulations.

==> Sections/trade-off.tex <==
%!TEX ROOT = ../collaboration_vs_competition.tex

\subsection{Competition-Collaboration Trade-Off: an Analytical Insight}\label{sec:trade-off}

The analytical expression of the consensus error %~\eqref{eq:cons-error-regular}
is hard to parse, through the presence of the trace operator
and the fact that it is not possible to characterize the spectrum of the trace argument,
nor the latter can be cast as a semi-definite matrix.

Yet, some intuition can be achieved from the following decomposition. % suitably the error function.
Assuming that there is one malicious \node $ m $, $ \malSet = \{m\} $,
and that the covariance matrix $ \Varn $ is diagonal,
from~\eqref{eq:cons-error-regular-all-priors} we can expand the error as follows,
\begin{equation}\label{eq:cons-error-regular-split}
	\ereg = \underbrace{\left(\varnode{m}+d\right)\left\| L_m^{-m}\right\|^2}_{e_{\regSet,\mathrm{collaboration}}} \: + \:
	\underbrace{\sumreg{i}\varnode{i}\left\| L_i^{-m} - \dfrac{\one}{R}\right\|^2}_{e_{\regSet,\mathrm{competition}}} ,
\end{equation}
where $ L_i\in\Real{N} $ is the $ i $th column of $ L $
and $ L_i^{-m}\in\Real{R} $ is obtained from $ L_i $ by removing its $ m $th row.
The error curve together with its two addends are shown in~\autoref{fig:trade-off}.
Equation~\eqref{eq:cons-error-regular-split} allows for an intuitive interpretation of the error,
which leverages the notion of \textit{social power} in opinion dynamics.

In social networks, the social power is used to quantify how much each agent's
opinion affects the opinion of all agents.
In particular, when opinions evolve according to the FJ dynamics,
the element $ L_{ij} $ quantifies the influence of 
%the initial opinion of 
agent $ j $ on agent $ i $:
as $ L_{ij} $ increases,
agent $ i $ is more affected by agent $ j $'s initial opinion.
The overall social power of agent $ j $ is a symmetric and increasing function of all elements $ L_{ij} $, $ i\in\sensSet $.%
\footnote{For example,~\cite{cartwright1959studies} defines it as the arithmetic mean of $ \{L_{ij}\}_{j=1}^N $.}

\begin{figure}
	\centering
	\includegraphics[width=.8\linewidth]{trade-off}
	\caption{Cost contributions in~\eqref{eq:cons-error-regular-split}.}
	\label{fig:trade-off}
\end{figure}

Borrowing such concepts from opinion dynamics
allows us to interpret the two contributions adding up in~\eqref{eq:cons-error-regular-split}.
The first contribution, $ e_{\mathcal{R},\mathrm{collaboration}} $,
quantifies the impact of the malicious \node on regular \nodes.
In particular, the \textquotedblleft social power" of $ m $, % on the regular agents,
as quantified by the norm of $ L_{m}^{-m} $,
depends on the communication graph and on the parameter $ \lam $.
In fact, each element of $ L_{m}^{-m} $ decreases with $ \lam $
because the malicious \node's influence diminishes as the regular \nodes anchor more tightly to their priors.
This can be proved by noting (cf.~\eqref{eq:M-block-matrix})
\begin{equation}\label{eq:L_im-decreasing}
	\dfrac{dL}{d\lam} = \dfrac{1}{\lam}L\left(I-WL\right) \ \rightarrow \ \dfrac{dL_{im}}{d\lam} < 0, \, i\in\regSet.
\end{equation}

The second contribution,  $ e_{\mathcal{R},\mathrm{competition}} $,
is a measure of how \textquotedblleft democratic" the interaction among regular \nodes is:
\ie it is proportional to the mismatch between how much each regular \node affects the others
and the ideal value $ \nicefrac{1}{R} $,
which means that each \node affects all \nodes equally.
%and that influence happens only within the set of regular \nodes.
Such a cost is zero only if the submatrix of $ L $
describing the interactions among regular \nodes is the consensus matrix: %equal to $ \Creg $:
this can happen only if %the associated submatrix of $ W $ is doubly stochastic
the regular \nodes do not interact with the malicious~\cite{7577815}.
In this special case,
$ e_{\mathcal{R},\mathrm{competition}} $ is zero at $ \lam = 0 $
and increases monotonically as the network shifts
from a democratic system, where all \nodes affect each other equally ($ \lam = 0 $),
to a disconnected system where \nodes cannot affect each other ($ \lam = 1 $).
In the case with malicious \nodes,
$ e_{\mathcal{R},\mathrm{competition}} $ exhibits a U-shape.
For small $ \lam $,
the malicious \node rules the overall dynamics,
and interactions among regular \nodes are negligible.
As $ \lam $ increases, the regular \nodes start collaborating %are less affected by the malicious \node,
and their interactions become closer to democracy, making$ e_{\mathcal{R},\mathrm{competition}} $ decrease.
However, as $ \lam $ grows further,
regular \nodes stick to their priors
%and do not let other \nodes becomes too weak,
and set themselves isolated from others. % and get farther away from the democratic system.
In practice, numerical tests show that the point of minimum of $ e_{\mathcal{R},\mathrm{competition}} $
is small (see zoomed box in~\autoref{fig:trade-off}).

%so that the increasing branch of the curve involves most values of $ \lam $.
Overall, %according to intuition,
%we conclude that 
the error has two concurrent causes that generate a phase transition:
the collaboration with the malicious \node is critical for small $ \lam $,
while for large $ \lam $ the error is mainly due to \nodes competing too aggressively, % each other.
rejecting possibly useful shared information.
In fact, this analysis matches intuition from~\eqref{eq:FJ-dynamics},
where $ \lam $ measures conservatism in \node updates.
